vContact: Private WiFi-based Contact Tracing with Virus Lifespan

Covid-19 is primarily spread through contact with the virus which may survive on surfaces with lifespan of more than hours. To curb its spread, it is hence of vital importance to detect and quarantine those who have been in contact with the virus for sustained period of time, the so-called close contacts. In this work, we study, for the first time, automatic contact detection when the virus has a lifespan. Leveraging upon the ubiquity of WiFi signals, we propose a novel, private, and fully distributed WiFi-based approach called vContact. Users installing an app continuously scan WiFi and store its hashed IDs. Given a confirmed case, the signals of the major places he/she visited are then uploaded to a server and matched with the stored signals of users to detect contact. vContact is not based on phone pairing, and no information of any other users is stored locally. The confirmed case does not need to have installed the app for it to work properly. As WiFi data are sampled sporadically, we propose efficient signal processing approaches and similarity metric to align and match signals of any time. We conduct extensive indoor and outdoor experiments to evaluate the performance of vContact. Our results demonstrate that vContact is efficient and robust for contact detection. The precision and recall of contact detection are high (in the range of 50-90%) for close contact proximity (2m). Its performance is robust with respect to signal lengths (AP numbers) and phone heterogeneity. By implementing vContact as an app, we present a case study to demonstrate the validity of our design in notifying its users their exposure to virus with lifespan.

==> 3-1_Summary.tex <==
\section{Summary}
\label{sec: summary}


Covid-19
%has cost us dearly valuable lives and the global economy. It
is primarily spread through contact with the virus which, according to some studies, may survive on surfaces with lifespan of more than hours.
To curb its spread, it is hence
of vital importance to detect and quarantine those who have been in contact with the virus for sustained period of time, the so-called {\em close contacts}.
%Study has shown that the virus has certain lifespan on surfaces, ranging from hours to days. People coming into contact with the virus for
%sustained period of time would be at risk.
The existing digital approaches for contact tracing focuses only on direct face-to-face contacts. There has not been any work detecting indirect environmental contact as well,
%virus lifespan,
that is to detect people coming into an area with living virus, i.e., an area 
previously visited by an infected person within the virus lifespan.

In this work, we study, for the first time, automatic contact detection when the virus has a lifespan. Leveraging upon the ubiquity of WiFi signals, we propose a novel, private, and fully distributed WiFi-based approach called \sysname{}.
%to detect close contacts.
%To the best of our knowledge, this is the first piece of work considering the virus lifespan in private contact tracing. Note that though our discussion is on WiFi, our approach can be equally extended and applied to other radio-frequenccy signals (such as bluetooth) and their combination.
Users installing an app continuously scan WiFi and stores its hashed IDs.  Given a confirmed case, the signals of the major places he/she visited are then uploaded to a server and  matched with the the stored signals of users to detect contact.  \sysname{} is not based on phone pairing, and no information of any other users is stored locally.  The confirmed case does not need to have installed the app for it to work properly.
As WiFi data are sampled sporadically, we 
propose efficient signal processing approaches and 
similarity metric to align and match signals of any time.
%contact detection, considering the overlap ratio of signals and their strength difference.
We conduct extensive indoor and outdoor experiments to evaluate the performance of \sysname{}. Our results demonstrate that \sysname{} is efficient and robust for contact detection. The precision and recall of contact detection are high (in the range of 50--90\%)
%$72\% \sim 79\%$  and $71\% \sim 87\%$)
for close contact proximity ($2$m). Its performance is robust with respect to signal lengths (AP numbers) and phone heterogeneity. By implementing \sysname{} as an app, we present a case study to demonstrate the validity our design in notifying its users their exposure to virus
%close contact detection
with lifespan.


%In our work, we propose solutions for two case, confirmed cases with APP and without APP. 


==> algorithm/direct_contact_tracing.tex <==
\SetArgSty{textnormal}
\let\oldnl\nl% Store \nl in \oldnl
\newcommand{\nonl}{\renewcommand{\nl}{\let\nl\oldnl}}% Remove line number for one line
\begin{algorithm2e}
\SetAlgoLined


\textbf{Input}: A normal user's WiFi data W ;  \\
\nonl \hspace*{10mm} An infected user's WiFi data $\hat{W}$;  \\
\nonl \hspace*{10mm} A proximity threshold $\theta$. \\

\textbf{Output}: results of direct contact detection  at different timestamp in $W$.
\BlankLine
Initialize $S$ to empty; \\
Construct the WiFi profile of the path F from $\hat{W}$;\\

\ForEach{($A_i, t_i) \in W$}
{
    initialize $s = 0$;\\
    \ForEach{$(\hat{A}_j,T_j) \in F$}
    {
        \If{$t_i \in T_j$} 
        {
            $s = P(A_i, \hat{A}_j)$;\\
            \uIf{$s > \theta$}
            {
                Append $(True,t_i)$ to $S$;
            }
           \uElse
            {
                Append $(False,t_i)$ to $S$;
            }
            
            break;
        }
        
    }
}

\textbf{return} $S$


\caption{Contact Detection}
\label{algo_direct_tracing}
\end{algorithm2e}
